On the Robustness of Deep Learning-predicted Contention Models for Network Calculus

The network calculus (NC) analysis takes a simple model consisting of a network of schedulers and data flows crossing them. A number of analysis "building blocks" can then be applied to capture the model without imposing pessimistic assumptions like self-contention on tandems of servers. Yet, adding pessimism cannot always be avoided. To compute the best bound on a single flow's end-to-end delay thus boils down to finding the least pessimistic contention models for all tandems of schedulers in the network - and an exhaustive search can easily become a very resource intensive task. The literature proposes a promising solution to this dilemma: a heuristic making use of machine learning (ML) predictions inside the NC analysis. While results of this work were promising in terms of delay bound quality and computational effort, there is little to no insight on when a prediction is made or if the trained algorithm can achieve similarly striking results in networks vastly differing from its training data. In this paper, we address these pending questions. We evaluate the influence of the training data and its features on accuracy, impact and scalability. Additionally, we contribute an extension of the method by predicting the best $n$ contention model alternatives in order to achieve increased robustness for its application outside the training data. Our numerical evaluation shows that good accuracy can still be achieved on large networks although we restrict the training to networks that are two orders of magnitude smaller.

==> include/robustness.tex <==
% !TeX root = ../ms.tex
% !TeX encoding = UTF-8
% !TeX spellcheck = en_US

\section{Increasing the Robustness of DeepTMA}
\label{sec:robustness}

We describe in this section our extension of DeepTMA for generating multiple tandem decompositions as well as our dataset generation process.

\subsection{DeepTMA\textsubscript{$n$}: Generate multiple tandem decompositions}
\label{sec:graphnn:multiple}

Given a foi and a potential cut location, the output of the neural network is a probability of cutting.
This probability is generated by the neural network using the softmax function after its last layer.
In case a single tandem decomposition has to be generated, the decision of cutting is made using a threshold of \SI{50}{\percent}.

Those cut probabilities may also be used in order to generate multiple tandem decompositions as illustrated in \cref{algo:multipletandems}.
In case the number of tandem decompositions is lower than the number of requested decompositions, we simply return all combinations of cuts.
Otherwise, we sample the distribution of cuts in order to generate the decompositions.
We label this extension of DeepTMA as DeepTMA\textsubscript{$n$}, with $n$ the number of tandem decompositions generated.

\begin{algorithm}[h!]
	\caption{Generation of $n$ tandem decompositions for a flow traversing $L+1$ servers.}
	\label{algo:multipletandems}
	\begin{algorithmic}
		\If{$n \leq L^2$}
			\Return all combinations of cuts
		\Else
			\ForAll{$i := 1$ \textbf{to} $n$}
				\State $v \gets [c_1, \ldots, c_{L}] \sim \mathcal{U}(0, 1)^{L}$
				\State cuts\textsubscript{$i$} $\gets \mathbb{I}\left( v \leq \left[ \Pr(\mathit{cut}_{foi, 1}^{GNN}), \ldots, \Pr(\mathit{cut}_{foi, L}^{GNN}) \right] \right)$
				\State \hspace{10pt} ($\mathbb{I}$ is the indicator function)
			\EndFor
			\Return \{cuts\textsubscript{$1$}, \ldots, cuts\textsubscript{$n$}\}
		\EndIf
	\end{algorithmic}
\end{algorithm}


\subsection{Dataset generation}
\label{sec:dataset_generation}

In order to train our neural network architecture, we randomly generated a set of topologies according to three different random topology generators:
\begin{enumerate*}[label=\textit{\alph*)}]
	\item tandems or daisy-chains,
	\item trees and
	\item random server graphs following the $G(n,p)$ Erdős–Rényi model~\cite{Erdos1959}.
\end{enumerate*}
For each created server, a rate latency service curve was generated with uniformly random rate and latency parameters.
A random number of flows with random source and sink servers was added. 
Note that in our topologies, there cannot be cyclic dependency between the flows.
For each flow, a token bucket arrival curve was generated with uniformly random burst and rate parameters.
All curve parameters were normalized to the $(0, 1]$ interval.

In total, \num{172374} different networks were generated, with a total of more than 13 million flows, and close to 260 million tandem decompositions.
Half of the networks were used for training the neural network, while the other half was used for the evaluation presented later in \Cref{sec:evaluation}.
\Cref{tab:dataset_stats} summarizes different statistics about the generated dataset.
The dataset is will be available online to reproduce our learning results.
Note that compared to the original dataset used for training DeepTMA \cite{Geyer2019}, this dataset contains larger networks.

\begin{table}[h!]
	\centering
	\resizebox{%
		\ifdim\width>\columnwidth
		\columnwidth
		\else
		\width
		\fi
	}{!}{%
	\begin{tabular}{@{}l|rrrr@{}}
		\toprule
		\textbf{Parameter}                & \quad\textbf{Min} & \quad\quad\textbf{Max} & \quad\textbf{Mean} & \textbf{Median} \\ \midrule
		\# of servers                     &            2 &           41 &          14.6 &              12 \\
		\# of flows                       &            3 &          203 &         101.2 &             100 \\
		\# of tandem combinations         &            2 & \num{197196} &  \num{1508.5} &             384 \\
		\# of nodes in analyzed graph     &           10 &   \num{2093} &         545.2 &             504 \\
		\# of tandem combination per flow &            2 &  \num{65536} &          19.4 &               4 \\
		\# of flows per server            &            1 &          173 &          18.1 &              10 \\ \bottomrule
	\end{tabular}}
	\caption{Statistics about the randomly generated dataset.}
	\label{tab:dataset_stats}
\end{table}


Additionally to this dataset, we also evaluate our approach on the set of networks used in \cite{Bondorf2017a}.
\Cref{tab:dataset_stats_pomacs2017} summarizes different statistics about the generated dataset.
Compared to dataset used for training, this additional set of networks up to two order of magnitude larger in term of number of servers and flows per network.
This property will be used in \cref{sec:evaluation} in order to evaluate if our approach is able to scale to such larger networks, both in term of accuracy and execution time.

\begin{table}[h!]
	\centering
	\resizebox{%
		\ifdim\width>\columnwidth
		\columnwidth
		\else
		\width
		\fi
	}{!}{%
	\begin{tabular}{@{}l|rrrr@{}}
		\toprule
		\textbf{Parameter}                & \quad\textbf{Min} & \quad\quad\textbf{Max} & \quad\textbf{Mean} & \textbf{Median} \\ \midrule
		\# of servers                     &           38 &   \num{3626} &         863.0 &             693 \\
		\# of flows                       &          152 &  \num{14504} &  \num{3452.0} &      \num{2772} \\
		\# of tandem combinations         &   \num{2418} & \num{121860} & \num{24777.6} &     \num{18869} \\
		\# of nodes in analyzed graph     &   \num{1358} & \num{113162} & \num{25137.7} &     \num{19518} \\
		\# of tandem combination per flow &            2 &          512 &           7.3 &               8 \\
		\# of flows per server            &            1 &          467 &          16.4 &              12 \\ \bottomrule
	\end{tabular}}
	\caption{Statistics about the set of networks from \cite{Bondorf2017a}.}
	\label{tab:dataset_stats_pomacs2017}
\end{table}

